LeMMINGs. III. The e-MERLIN Legacy Survey of the Palomar sample. Exploring the origin of nuclear radio emission in active and inactive galaxies through the [O III] -- radio connection

What determines the nuclear radio emission in local galaxies? We combine optical [O III] line emission, robust black hole (BH) mass estimates, and high-resolution e-MERLIN 1.5-GHz data, from the LeMMINGs survey, of a statistically-complete sample of 280 nearby, optically active (LINER and Seyfert) and inactive HII and Absorption line galaxies [ALG]) galaxies. Using [O III] luminosity ($L_{\rm [O~III]}$) as a proxy for the accretion power, local galaxies follow distinct sequences in the optical-radio planes of BH activity, which suggest different origins of the nuclear radio emission for the optical classes. The 1.5-GHz radio luminosity of their parsec-scale cores ($L_{\rm core}$) is found to scale with BH mass ($M_{\rm BH}$) and [O~III] luminosity. Below $M_{\rm BH} \sim$10$^{6.5}$ M$_{\odot}$, stellar processes from non-jetted HII galaxies dominate with $L_{\rm core} \propto M_{\rm BH}^{0.61\pm0.33}$ and $L_{\rm core} \propto L_{\rm [O~III]}^{0.79\pm0.30}$. Above $M_{\rm BH} \sim$10$^{6.5}$ M$_{\odot}$, accretion-driven processes dominate with $L_{\rm core} \propto M_{\rm BH}^{1.5-1.65}$ and $L_{\rm core} \propto L_{\rm [O~III]}^{0.99-1.31}$ for active galaxies: radio-quiet/loud LINERs, Seyferts and jetted HII galaxies always display (although low) signatures of radio-emitting BH activity, with $L_{\rm 1.5\, GHz}\gtrsim$10$^{19.8}$ W Hz$^{-1}$ and $M_{\rm BH}\gtrsim10^{7}$ M$_{\odot}$, on a broad range of Eddington-scaled accretion rates ($\dot{m}$). Radio-quiet and radio-loud LINERs are powered by low-$\dot{m}$ discs launching sub-relativistic and relativistic jets, respectively. Low-power slow jets and disc/corona winds from moderately high to high-$\dot{m}$ discs account for the compact and edge-brightened jets of Seyferts, respectively. Jetted HII galaxies may host weakly active BHs. Fuel-starved BHs and recurrent activity account for ALG properties. [abridged]

==> binhex.tex <==
%%
%% This is file `binhex.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% binhex.dtx  (with options: `style')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from binhex.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file binhex.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\edef\next{\toks0=%
   {\catcode`\noexpand\@=\the\catcode`\@\toks0{\the\toks0}}%
}
\next
\catcode`\@11
\def\next#1#2#3{\expandafter \def \csname bb@#1\endcsname##1%
  {#2\csname bb@#3##1\endcsname}}
\next{00}00 \next{01}01 \next{02}10 \next{03}11
\next{04}20 \next{05}21 \next{06}30 \next{07}31
\next{08}40 \next{09}41 \next{10}50 \next{11}51
\next{12}60 \next{13}61 \next{14}70 \next{15}71
\next{16}80 \next{17}81 \next{18}90 \next{19}91
\expandafter \def \csname bb@0+\endcsname {+0}
\expandafter \def \csname bb@1+\endcsname {+1}
\def\bb@endbinary#1+{\fi\fi}
\expandafter \def \csname bb@0-\endcsname {0+-\bb@dobinary}
\expandafter\def\csname bb@0m\endcsname#1+{#1+0}
\expandafter\def\csname bb@1m\endcsname#1+{#1+1}
\def\bb@dobinary#1#2{\if#10\if m\string#2\else\bb@endbinary\fi\fi
 \expandafter\bb@dobinary\number\csname bb@0#1\endcsname#2}
\def\nbinary#1#2{\expandafter\bb@dobinary\number\number#2%
 \romannumeral\number\number#1 000+}
\def\binary{\nbinary1}
\def \next #1#2{\expandafter \def
 \csname bb@h\number +#1\endcsname ##1+{\bb@dohex ##1+#2}%
}
\next   {0}0 \next   {1}1 \next  {10}2 \next  {11}3
\next {100}4 \next {101}5 \next {110}6 \next {111}7
\next{1000}8 \next{1001}9 \next{1010}A \next{1011}B
\next{1100}C \next{1101}D \next{1110}E \next{1111}F
\def\bb@dohex #1{\csname bb@x#1\endcsname}
\def\bb@x\endcsname#1{ \bb@xm{m\endcsname}}
\def\bb@xm #1\endcsname #2#3+{#2#3%
 \csname bb@h\number+\endcsname
 #1\endcsname m#3+}
\def\bb@nbinbased #1#2#3{\expandafter \bb@dobinary \number#1%
 \expandafter \bb@dohex
 \romannumeral \number\number #2 000\expandafter\endcsname
 \romannumeral \number\number #3 000+}
\def\nbinbased #1#2#3{\expandafter\bb@nbinbased
 \expandafter {\number#3}{#2}{#1}}
\def\nhex{\nbinbased4}
\def\noct{\nbinbased3}
\def\ntetra{\nbinbased2}
\def\hex{\nhex1}
\def\oct{\noct1}
\def\tetra{\ntetra1}
\the\toks0
\endinput
%%
%% End of file `binhex.tex'.


==> opt_tab.tex <==
\onecolumn
\begin{center}
%\begin{longtable}{lC{1.85cm}C{2cm}C{0.3cm}ccC{1.8cm}C{1.7cm}C{0.8cm}cC{0.5cm}}
\begin{longtable}{lccC{0.4cm}C{3cm}cccccc}
\caption[Properties of the  sample.]{Optical-radio properties of the sample.} 
\label{bigtab} \\

%This is the header for the first page of the table...
\hline 
\hline
Name &  RA & DEC & D & Hubble    & class  & class  & $\sigma$   & M$_{\rm BH}$ & L$_{\rm [OIII]}$ &  Edd \\
     &     &    & Mpc& type     &    Ho97  &  BPT   &  km s$^{-1}$ &  M$_{\odot}$  & erg s$^{-1}$  & ratio \\
 (1) & (2)& (3) & (4)  & (5) & (6)      & (7)& (8) & (9) & (10)  & (11) \\    
\hline	
\endfirsthead


%This is the header for the remaining page(s) of the table...
\multicolumn{3}{c}{{\tablename} \thetable{} -- Continued} \\[0.5ex]
\hline
\hline
Name &  RA & DEC & D & Hubble    & class  & class  & $\sigma$   & M$_{\rm BH}$ & L$_{\rm [OIII]}$ &  Edd \\
     &     &    & Mpc& type     &  Ho97 &  BPT   &  km s$^{-1}$ &  M$_{\odot}$  & erg s$^{-1}$  &    ratio \\
 (1) & (2)& (3) & (4)  & (5) & (6)      & (7)& (8) & (9) & (10)  & (11) \\   
\hline 

\endhead


%This is the footer for all pages except the last page of the table...
\hline
  \multicolumn{11}{c}{{Continued on Next Page}} \\
\endfoot


%This is the footer for the last page of the table...
 \\[-1.8ex] 
\endlastfoot

%Now the data...
NGC~783  &    02 01 06.61 &    +31 52 56.8 &       68.1 & SAc             &             H & H             & 101.4 & 6.94             & 38.81    & $-$2.68   \\                 
IC~239   &    02 36 27.82 &    +38 58 09.1 &       16.8 & SAB(rs)cd       &         L2::  & H$^{a}$        & 92.3  & 6.78            & $<$36.93    & $<$$-$4.40  \\          
NGC~1003 &    02 39 17.03 &    +40 52 21.3 &       10.7 & SA(s)cd         &           ALG & H$^{b,c}$      & -     & -               & 37.23    & $-$       \\                 
NGC~1023 &    02 40 24.01 &    +39 03 47.7 &       10.5 & SB(rs)0-        &           ALG &  ALG$^{b}$     & 204.5 & 7.62$^{*}$      & $-$      & $-$      \\                  
NGC~1058 &    02 43 30.01 &    +37 20 28.7 &        9.1 & SA(rs)c         &            S2 & L              & 31    & 4.88            & 35.95    & $-$3.48 \\                   
NGC~1156 &    02 59 42.85 &    +25 14 28.4 &        6.4 & IB(s)m          &             H & H              & 35.9  & 5.13            & 39.15    & $-$0.53   \\                 
NGC~1161 &    03 01 14.17 &    +44 53 50.7 &       25.9 & SA0             &         T1.9: &  L             & 258.4 & 8.58            & 38.13    & $-$5.00  \\                  
NGC~1167 &    03 01 42.34 &    +35 12 19.9 &       65.3 & SA0-            &            S2 &  L             & 216.9 & 8.27            & 40.17    & $-$2.65   \\                 
NGC~1169 &    03 03 34.76 &    +46 23 10.7 &       33.7 & SAB(r)b         &          L2   &  L$^{d}$        & 181.3 & 7.96           & 38.58    & $-$3.93  \\                  
NGC~1186 &    03 05 30.85 &    +42 50 07.7 &       35.4 & SB(r)bc:        &            H  & H              & 119.8 & 7.24            & 38.95    & $-$2.84   \\                 
NGC~1275 &    03 19 48.16 &    +41 30 42.1 &       70.1 & Pec             &         S1.5  & L$^{e}$         & 258.9 & 8.98$^{*}$      & 41.61    & $-$1.92  \\                 
IC~342   &    03 46 48.51 &    +68 05 46.0 &        3.0 & SAB(rs)cd       &           H   & H               & 74.0  & 6.41$^{*}$      & 35.99 & $-$4.97   \\                   
IC~356   &    04 07 46.88 &    +69 48 44.7 &       18.1 & SA(s)ab pec     &            T2 & H$^{b}$         & 156.6 & 7.70            & 37.57    & $-$4.68 \\                  
NGC~1569 &    04 30 49.19 &    +64 50 52.5 &        1.6 & IBm             &           H   & H               & 44    & 5.49           & 36.49 & $-$3.55   \\                    
NGC~1560 &    04 32 49.09 &    +71 52 59.2 &        3.0 & SA(s)d spin     &           H   & H               & 33.9  & 5.03           & 37.38    & $-$2.20  \\                  
NGC~1961 &    05 42 04.61 &    +69 22 42.3 &       53.1 & SAB(rs)c        &            L2 &  L$^{f}$        & 241.3 & 8.29$^{*}$      & 39.11    & $-$3.73 \\                 
NGC~2146 &    06 18 37.71 &    +78 21 25.3 &       17.2 & SB(s)ab pec     &           H   &  H              & 126.8 & 7.33           & 38.36    & $-$3.52   \\                 
UGC~3714 &    07 12 32.68 &    +71 45 01.9 &       40.9 & S? pec          &           H   & H               & 104   & 6.99           & 38.49    & $-$3.05   \\                 
NGC~2336 &    07 27 03.66 &    +80 10 42.0 &       33.9 & SAB(r)bc        &         L2/S2 &  L              & 116.2 & 7.18           & 38.20    & $-$3.54   \\                 
NGC~2366 &    07 28 51.85 &    +69 12 31.1 &        2.9 & IB(s)m          &           ALG & H$^{f,g}$        & $-$   & $-$            & $-$      & $-$     \\                  
IC~467   &    07 30 18.40 &    +79 52 21.1 &       27.4 & SAB(s)c:        &           H:  &  H              & 64.2  & 6.15           & 37.15    & $-$3.55  \\                  
NGC~2403 &    07 36 51.40 &    +65 36 09.2 &        4.2 & SAB(s)cd        &           H   &  H:$^{f}$        & 68.4  & 6.26           & $<$35.91    & $<$$-$4.90  \\        
NGC~2549 &    08 18 58.35 &    +57 48 10.9 &       18.8 & SA(r)0 spin     &           ALG & ALG$^{f}$        & 142.6 & 7.16$^{*}$     & $-$      & $-$      \\                 
NGC~2683 &    08 52 41.35 &    +33 25 18.5 &        5.7 & SA(rs)b         &         L2/S2 & L               & 130.2 & 7.38           & 37.06    & $-$4.87   \\                 
NGC~2685 &    08 55 34.75 &    +58 44 03.9 &       16.2 & (R)SB0+pec      &        S2/T2: & L               & 93.8  & 6.59$^{*}$      & 38.41    & $-$2.73  \\                 
NGC~2750 &    09 05 47.89 &    +25 26 14.5 &       38.4 & SABc            &           H   & H               & 52.4  & 5.79            & 39.20    & $-$1.14   \\                
NGC~2742 &    09 07 33.58 &    +60 28 45.8 &       22.2 & SA(s)c:         &           H   & H               & 65.6  & 6.18            &  37.73    & $-$3.00  \\                
NGC~2770 &    09 09 33.62 &    +33 07 24.3 &       29.6 & SA(s)c:         &           H   & H               & 81    & 6.55            & 37.56    & $-$3.54  \\                 
NGC~2768 &    09 11 37.50 &    +60 02 14.8 &       23.7 & E6:             &         L2    & L$^{g}$         & 181.8 & 7.96            & 38.61    & $-$3.90  \\                 
NGC~2776 &    09 12 14.53 &    +44 57 17.6 &       38.7 & SAB(rs)c        &         H     & H               & 47.7  & 5.63            & 38.32    & $-$1.86   \\                
NGC~2782 &    09 14 05.12 &    +40 06 49.1 &       37.3 & SAB(rs)a pec    &         H     & H               & 183.1 & 7.98            & 40.00    & $-$2.53   \\                
NGC~2787 &    09 19 18.54 &    +69 12 11.6 &       13.0 & SB(r)0+         &         L1.9  & L               & 202   & 7.61$^{*}$      & 38.37    & $-$3.79   \\               
NGC~2832 &    09 19 46.88 &    +33 44 59.4 &       91.6 &  E+2:           &         L2::  & L$^{b}$         & 334   & 9.03             & $<$39.05  & $<$$-$4.53  \\            
NGC~2859 &    09 24 18.53 &    +34 30 47.5 &       25.4 & (R)SB(r)0+      &         T2:   & L               & 188.2 & 8.02             & 38.57    & $-$4.00  \\                
NGC~2903 &    09 32 10.11 &    +21 30 03.0 &        6.3 & SAB(rs)bc       &           H   & H               & 89    & 7.06$^{*}$       & 37.35    & $-$4.26   \\               
NGC~2950 &    09 42 35.12 &    +58 51 04.4 &       23.3 & (R)SB(r)0       &           ALG & ALG             & 163   & 7.77             & $-$      & $-$     \\                 
NGC~2964 &    09 42 54.23 &    +31 50 50.2 &       21.9 & SAB(r)bc:       &           H   & H               & 109.4 & 6.73$^{*}$       & 38.71    & $-$2.57   \\               
NGC~2977 &    09 43 46.80 &    +74 51 34.9 &       40.9 & SAb:            &           H   & H               & 104.5 & 7.00             & 38.20    & $-$3.35  \\                
NGC~2976 &    09 47 15.46 &    +67 54 59.0 &        2.1 & SAc pec         &           H   & H               & 36    & 5.14             & 36.58    & $-$3.11  \\                
NGC~3003 &    09 48 36.05 &    +33 25 17.4 &       24.4 & SAbc?           &           H   & H               & 44.1  & 5.49             & 38.90    & $-$1.14  \\                
NGC~2985 &    09 50 22.23 &    +72 16 4.0 &       22.4 &  R')SA(rs)ab    &         T1.9   & L$^{h}$         & 140.8 & 7.52            & 38.69    & $-$3.38  \\                
NGC~3031 &    09 55 33.17 &    +69 03 55.1 &        1.4 & SA(s)ab         &         S1.5  & L$^{f,g,h}$      & 161.6 & 7.81$^{*}$       & 37.72    & $-$4.64  \\               
NGC~3027 &    09 55 40.63 &    +72 12 12.8 &       19.5 & SB(rs)d:        &           H   & H               & 25.6  & 4.54             & 37.69    & $-$1.40   \\               
NGC~3034 &    09 55 52.43 &    +69 40 46.9 &        5.2 & IAO spin        &           H   & H               & 129.5 & 7.37             & 38.33   & $-$3.59  \\                   
NGC~3043 &    09 56 14.85 &    +59 18 25.6 &       39.1 & SAb: spin       &           H   & H               & 51.9  & 5.77             & 38.08    & $-$2.24   \\               
NGC~3073 &    10 00 52.20 &    +55 37 07.9 &       19.3 & SAB0-           &           H   & H$^{i}$         & 35.6  & 5.12             & 38.02    & $-$1.65  \\                
NGC~3077 &    10 03 19.10 &    +68 44 1.6 &        2.1 &  AO pec         &           H    & H               & 32.4  & 4.95             & 37.15    & $-$2.35 \\                
NGC~3079 &    10 01 57.80 &    +55 40 47.2 &       20.4 & SB(s)c spin     &         S2    & L$^{i}$         & 182.3 & 6.40$^{*}$        & 37.67    & $-$3.28 \\                   
NGC~3162 &    10 13 31.59 &    +22 44 15.2 &       22.2 & SAB(rs)bc       &           H   & H               & 89    & 6.72             & 38.04    & $-$3.23  \\                
NGC~3147 &    10 16 53.62 &    +73 24 02.3 &       40.9 & SA(rs)bc        &       S2      & L               & 219.8 & 8.29             & 39.54    & $-$3.30   \\               
NGC~3185 &    10 17 38.56 &    +21 41 17.8 &       21.3 & (R)SB(r)0/a     &       S2:     & S               & 79.3  & 6.51             & 39.44    & $-$1.62   \\               
NGC~3190 &    10 18 05.63 &    +21 49 55.6 &       22.4 & SA(s)a pec spin &         L2    & L               & 188.1 & 8.02             & 38.71    & $-$3.86   \\               
NGC~3193 &    10 18 24.88 &    +21 53 38.3 &       23.2 & E2              &         L2:   & L               & 194.3 & 8.08             & 38.42    & $-$4.21   \\               
NGC~3245 &    10 27 18.39 &    +28 30 26.8 &       22.2 & SA(r)0?         &         T2:   & H$^{i}$          & 209.9 & 8.38$^{*}$      & 38.70    & $-$4.23   \\              
IC~2574  &    10 28 23.62 &    +68 24 43.4 &        3.4 & SAB(s)m         &           H   & H               & 33.9  & 5.03             & 35.55    & $-$4.03   \\               
NGC~3254 &    10 29 19.92 &    +29 29 39.2 &       23.6 & SA(s)bc         &       S2      & S               & 117.8 & 7.21             & 38.60    & $-$3.16   \\               
NGC~3301 &    10 36 56.03 &    +21 52 55.8 &       23.3 & (R')SB(rs)0/a   &         L2    & L$^{j}$         & 132.3 & 7.41             & $<$38.30 & $<$$-$3.66  \\                
NGC~3310 &    10 38 45.86 &    +53 30 11.9 &       18.7 & SAB(r)bc pec    &         H     & H               & 84    & 6.70$^{*}$       & 38.43    & $-$2.82  \\                  
NGC~3344 &    10 43 31.15 &    +24 55 20.0 &        6.1 & (R)SAB(r)bc     &         H     & H               & 73.6  & 6.38             & 38.24    & $-$2.69   \\               
NGC~3359 &    10 46 36.86 &    +63 13 27.3 &       19.2 & SB(rs)c         &           H   & H               & 55.3  & 5.89             & 37.36    & $-$3.08  \\                
NGC~3348 &    10 47 10.00 &    +72 50 22.8 &       37.8 & E0              &           ALG & ALG             & 236.4 & 8.42              & $-$      & $-$       \\              
NGC~3395 &    10 49 50.11 &    +32 58 58.3 &       27.4 & SAB(rs)cd: pec  &           H   & H               & 96.5  & 6.86             & 37.93   & $-$3.48 \\                  
NGC~3448 &    10 54 39.20 &    +54 18 17.5 &       24.5 & IAO             &           H   & H               & 50.7  & 5.73              & 39.48    & $-$0.80  \\               
NGC~3486 &    11 00 23.87 &    +28 58 30.5 &        7.4 & SAB(r)c         &       S2      & S               & 65    & 6.17             & 37.93    & $-$2.79   \\               
NGC~3504 &    11 03 11.21 &    +27 58 21.0 &       26.5 & (R)SAB(s)ab     &         H     & H               & 119.3 & 7.23             & 39.88    & $-$1.90   \\               
NGC~3516 &    11 06 47.49 &    +72 34 06.9 &       38.9 & (R)SB(s)0:      &       S1.2    & S               & 181   & 7.96             & 40.80    & $-$1.71  \\                
NGC~3556 &    11 11 30.97 &    +55 40 26.8 &       14.1 & SB(s)cd spin    &           H   &  H              & 79.4  & 6.52             & 37.62    & $-$3.45   \\               
NGC~3610 &    11 18 25.27 &    +58 47 10.6 &       29.2 & E5:             &           ALG & ALG             & 161.2 & 7.75             & $-$      & $-$      \\                
NGC~3613 &    11 18 36.11 &    +58 00 00.0 &       32.9 & E6              &           ALG & ALG             & 220.1 & 8.30             & $-$      & $-$      \\                
NGC~3631 &    11 21 02.87 &    +53 10 10.5 &       21.6 & SA(s)c          &           H   & H               & 43.9  & 5.48             & $<$38.01    & $<-$2.02  \\      
NGC~3646 &    11 21 43.08 &    +20 10 10.4 &       56.8 & Ring            &       H/T2:   & L               & 153.1 & 7.66             & 39.15    & $-$3.06   \\               
NGC~3642 &    11 22 17.89 &    +59 04 28.3 &       27.5 & SA(r)bc:        &         L1.9  & L$^{h}$          & 85    & 7.42$^{*}$       & 38.96    & $-$3.01  \\               
NGC~3690 &    11 28 32.30 &    +58 33 43.0 &       40.4 & IBm pec         &         H     & H               & 143.9 & 7.56             & 39.98    & $-$2.13   \\               
UGC~6484 &    11 29 11.76 &    +57 07 55.4 &       32.4 & SB(rs)c         &           H   & H               & 61.1  & 6.06             & 37.47    & $-$3.14   \\               
NGC~3718 &    11 32 34.85 &    +53 04 04.5 &       17.0 & SB(s)a pec      &         L1.9  & L$^{k}$          & 158.1 & 7.72             & 37.41    & $-$4.86 \\                
NGC~3729 &    11 33 49.32 &    +53 07 32.0 &       17.0 & SB(r)a pec      &           H   & H                & 76.2  & 6.45             & 36.60    & $-$4.40 \\                
NGC~3738 &    11 35 48.79 &    +54 31 26.0 &        4.3 & IAm             &           H   & H                & 49.1  & 5.68            & 37.77    & $-$2.46  \\                
NGC~3735 &    11 35 57.30 &    +70 32 08.1 &       41.0 & SAc: spin       &       S2:     & S                & 140.6 & 7.51            & 39.88    & $-$2.18   \\               
NGC~3756 &    11 36 48.02 &    +54 17 36.8 &       23.5 & SAB(rs)bc       &           H   & H                & 47.6  & 5.62            & 37.04    & $-$3.13  \\                
NGC~3780 &    11 39 22.36 &    +56 16 14.4 &       37.2 & SA(s)c:         &         L2::  & L$^{i}$          & 89.8  & 6.73            & 37.43    & $-$3.85  \\                
NGC~3813 &    11 41 18.66 &    +36 32 48.5 &       26.4 & SA(rs)b:        &           H   & H                & 72.1  & 6.35            &  37.59    & $-$3.31  \\               
NGC~3838 &    11 44 13.76 &    +57 56 53.6 &       24.6 & SA0/a?          &           ALG & ALG$^{k}$         & 141.4 & 7.52            & $-$      & $-$      \\               
NGC~3884 &    11 46 12.18 &    +20 23 29.9 &       91.6 & SA(r)0/a        &         L1.9  & L                & 208.3 & 8.20            & 40.20    & $-$2.55   \\               
NGC~3900 &    11 49 09.46 &    +27 01 19.3 &       29.4 & SA(r)0+         &         L2:   & ALG              & 139.2 & 7.50            & $<$38.35  & $<-$3.70  \\                
NGC~3898 &    11 49 15.37 &    +56 05 03.7 &       21.9 & SA(s)ab         &         T2    & L$^{b,k}$         & 206.5 & 8.19            & 38.52    & $-$4.03  \\               
NGC~3917 &    11 50 45.43 &    +51 49 28.8 &       17.0 & SAcd:           &         T2:   & L                & 38    & 5.23             & 36.90    & $-$2.88   \\              
NGC~3941 &    11 52 55.36 &    +36 59 10.8 &       18.9 & SB(s)0          &       S2:     & S$^{b}$           & 133   & 7.42            & 38.52    & $-$3.45  \\               
NGC~3945 &    11 53 13.73 &    +60 40 32.0 &       22.5 & (R)SB(rs)0+     &         L2    & L                & 191.5 & 6.94$^{*}$       & 38.39    & $-$3.10  \\               
NGC~3953 &    11 53 48.92 &    +52 19 36.4 &       17.0 & SB(r)bc         &         T2    & L                & 116   & 7.33$^{*}$       & 37.90    & $-$3.98   \\              
NGC~3963 &    11 54 58.71 &    +58 29 37.1 &       42.7 & SAB(rs)bc       &           H   & H                & 40.9  & 5.36             & 38.09    & $-$1.82  \\               
NGC~3982 &    11 56 28.13 &    +55 07 30.9 &       17.0 & SAB(r)b:        &       S1.9    & S                & 73    & 6.95$^{*}$       & 39.83    & $-$1.67   \\              
NGC~3992 &    11 57 35.98 &    +53 22 28.3 &       17.0 & SB(rs)bc        &         T2:   &  L$^{b,l}$        & 148.4 & 7.51$^{*}$      & 37.10 & $-$4.96 \\                  
NGC~3998 &    11 57 56.13 &    +55 27 12.9 &       21.6 & SA(r)0?         &         L1.9  & L                & 304.6 & 8.93$^{*}$       & 39.56 & $-$3.92 \\                   
NGC~4026 &    11 59 25.19 &    +50 57 42.1 &       17.0 & SA0 spin        &           ALG & L$^{b,m,n}$       & 177.2 & 8.26$^{*}$      & $-$      & $-$      \\              
NGC~4036 &    12 01 26.75 &    +61 53 44.8 &       24.6 & SA0-            &         L1.9  & L                & 215.1 & 7.89$^{*}$       & 39.16    & $-$3.28   \\              
NGC~4041 &    12 02 12.20 &    +62 08 14.0 &       22.7 & SA(rs)bc:       &         H     & H                & 95    & 6.83            & 38.24    & $-$3.14   \\              
NGC~4062 &    12 04 03.83 &    +31 53 44.9 &        9.7 & SA(s)c          &           H   & H                & 93.2  & 6.80             & 36.51    & $-$4.84  \\               
NGC~4088 &    12 05 34.19 &    +50 32 20.5 &       17.0 & SAB(rs)bc       &           H   & H                & 77    & 6.79$^{*}$       & 37.48    & $-$3.86   \\              
NGC~4096 &    12 06 01.13 &    +47 28 42.4 &        8.8 & SAB(rs)c        &           H   & H                & 79.5  & 6.52             & 36.15    & $-$4.92  \\               
NGC~4100 &    12 06 08.45 &    +49 34 57.7 &       17.0 & (R')SA(rs)bc    &           H   & H                & 75.5  & 6.43             &  37.95    & $-$3.03   \\             
NGC~4102 &    12 06 22.99 &    +52 42 39.9 &       17.0 & SAB(s)b?        &           H   & H                & 174.3 & 7.89             & 39.10    & $-$3.34   \\              
NGC~4111 &    12 07 03.13 &    +43 03 56.6 &       17.0 & SA(r)0+: spin   &         L2    & L                & 147.9 & 7.60             & 38.65    & $-$3.50   \\              
NGC~4125 &    12 08 06.02 &    +65 10 26.9 &       24.2 & E6 pec          &         T2    & L$^{b}$           & 226.7 & 8.35            & 38.71    & $-$4.19  \\               
NGC~4136 &    12 09 17.69 &    +29 55 39.4 &        9.7 & SAB(r)c         &           H   & H                & 38.4  & 5.25            & 37.39    & $-$2.41   \\               
NGC~4138 &    12 09 29.78 &    +43 41 07.1 &       17.0 & SA(r)0+         &         S1.9  & L                & 120.9 & 7.25            & 38.75    & $-$3.05   \\               
NGC~4143 &    12 09 36.06 &    +42 32 03.0 &       17.0 & SAB(s)0         &         L1.9  & L                & 204.9 & 7.92$^{*}$       & 38.81    & $-$3.66   \\              
NGC~4144 &    12 09 58.60 &    +46 27 25.8 &        4.1 & SAB(s)cd? spin  &           H   & H                & $<$64.3  & $<$6.15       & 36.26    & $>-$4.44   \\              
NGC~4145 &    12 10 01.52 &    +39 53 01.9 &       20.7 & SAB(rs)d        &         T2:   & H$^{i}$          & $-$   & 5.33$^{i}$        & 36.80    & $-$3.08     \\            
NGC~4151 &    12 10 32.58 &    +39 24 20.6 &       20.3 & (R')SAB(rs)ab:  &       S1.5    & S                & 97    & 7.81$^{*}$       & 41.74    &  $-$0.62     \\         
NGC~4150 &    12 10 33.65 &    +30 24 05.5 &        9.7 & SA(r)0?         &         T2    & L                & 87    & 5.94$^{*}$       & 35.83  & $-$-4.66 \\                  
NGC~4157 &    12 11 04.37 &    +50 29 04.8 &       17.0 & SAB(s)b? spin   &           H   &  H               & 90.1  & 6.74             & 36.96    & $-$4.33 \\                
NGC~4162 &    12 11 52.47 &    +24 07 25.2 &       38.5 & (R)SA(rs)bc     &           H   & H                & 76.1  & 6.44             & 38.44    & $-$2.55  \\               
NGC~4169 &    12 12 18.78 &    +29 10 45.9 &       50.4 & SA0             &       S2      & S                & 183   & 7.97              & 38.99    & $-$3.53  \\              
NGC~4183 &    12 13 16.88 &    +43 41 54.9 &       17.0 & SA(s)cd? spin   &           H   & H                & 34.4  & 5.06              & 37.90    & $-$1.71   \\             
NGC~4203 &    12 15 05.06 &    +33 11 50.4 &        9.7 & SAB0-:          &         L1.9  &  L               & 167   & 7.82$^{*}$        & 38.28   & $-$4.09 \\                   
NGC~4214 &    12 15 39.17 &    +36 19 36.8 &        3.5 & IAB(s)m         &           H   & H                & 51.6  & 5.76             & 38.71    & $-$1.60   \\              
NGC~4217 &    12 15 50.90 &    +47 05 30.4 &       17.0 & SAb spin        &           H   & H                & 91.3  & 6.76             & 36.93    & $-$4.38   \\              
NGC~4220 &    12 16 11.71 &    +47 52 59.7 &       17.0 & SA(r)0+         &          T2   & L                & 105.5 & 7.01              & 36.19    & $-$-5.37   \\            
NGC~4236 &    12 16 42.12 &    +69 27 45.3 &        2.2 & SB(s)dm         &           H   & H                & $<$62.8  &  $<$6.11           & 36.24    & $>-$4.42  \\       
NGC~4244 &    12 17 29.66 &    +37 48 25.6 &        3.1 & SA(s)cd: spin   &           H   & H                & 36.8  & 5.17             & 36.05    & $-$3.67   \\              
NGC~4242 &    12 17 30.18 &    +45 37 09.5 &        7.5 & SAB(s)dm        &           H:: & H:$^{i}$         & $-$   & $-$               & $<$36.30   &   $-$     \\              
NGC~4245 &    12 17 36.77 &    +29 36 28.8 &        9.7 & SB(r)0/a:       &           H   & H                & 82.7  & 7.19$^{*}$        & 37.36    & $-$4.38  \\              
NGC~4251 &    12 18 08.25 &    +28 10 31.4 &        9.7 & SB0? spin       &           ALG & ALG              & 119.4 & 7.23               & $-$      & $-$      \\             
NGC~4258 &    12 18 57.50 &    +47 18 14.3 &        6.8 & SAB(s)bc        &       S1.9    & S                & 148   & 7.58$^{*}$        & 38.76    & $-$3.37   \\             
NGC~4274 &    12 19 50.59 &    +29 36 52.1 &        9.7 & (R)SB(r)ab      &         H     & L$^{b,o}$         & 96.6  & 6.86              & 38.49    & $-$2.92  \\             
NGC~4278 &    12 20 06.82 &    +29 16 50.7 &        9.7 & E1+             &         L1.9 & L                 & 261   & 7.96$^{*}$        & 38.88    & $-$3.63   \\             
NGC~4291 &    12 20 18.20 &    +75 22 15.0 &       29.4 & E               &           ALG & ALG              & 285.3 & 8.99$^{*}$         & $-$      & $-$      \\             
NGC~4314 &    12 22 31.82 &    +29 53 45.2 &        9.7 & SB(rs)a         &         L2    & L$^{d,p}$         & 117   & 6.91$^{*}$        & 37.75    & $-$3.71   \\            
NGC~4346 &    12 23 27.94 &    +46 59 37.8 &       17.0 & SA0 spin        &         L2::  &  L$^{m}$         & 146.5 & 7.59               & 37.88    & $-$4.26  \\             
NGC~4369 &    12 24 36.20 &    +39 22 58.8 &       21.6 & (R)SA(rs)a      &           H   & H                & 71.6  & 6.34                & 38.83    & $-$2.06   \\           
NGC~4395 &    12 25 48.86 &    +33 32 48.9 &        3.6 & SA(s)m:         &       S1.8    & S                & 26    & 4.57                & 38.35    & $-$0.77  \\           
NGC~4414 &    12 26 27.10 &    +31 13 24.7 &        9.7 & SA(rs)c?        &         T2:   & L$^{b,c}$         & 117   & 7.19                 & 36.46    & $-$5.28 \\           
NGC~4449 &    12 28 11.10 &    +44 05 37.1 &        3.0 & IBm             &           H   & H                & 17.8  & 3.91                & 38.28    & $-$0.18   \\           
NGC~4448 &    12 28 15.43 &    +28 37 13.1 &        9.7 & SB(r)ab         &           H   & H                & 119.8 & 7.24                & 37.34    & $-$4.45   \\           
NGC~4460 &    12 28 45.56 &    +44 51 51.2 &        8.1 & SB(s)0+? spin   &           H   & H                & 39.8  & 5.31                  & 38.09    & $-$1.77   \\         
NGC~4485 &    12 30 31.13 &    +41 42 04.2 &        9.3 & IB(s)m pec      &           H   & H$^{q}$           & 52.2  & 5.78                & 36.95    & $-$3.38  \\           
NGC~4490 &    12 30 36.24 &    +41 38 38.0 &        7.8 & SB(s)d pec      &           H   & H$^{f,g}$          & 45.1  & 5.53                 & 37.12    & $-$-2.96  \\         
NGC~4494 &    12 31 24.10 &    +25 46 30.9 &        9.7 & E1+             &         L2::  & L$^{m}$           & 145   & 7.57               & 37.35    & $-$4.77  \\           
NGC~4559 &    12 35 57.65 &    +27 57 36.0 &        9.7 & SAB(rs)cd       &           H   & H                 & 49.2  & 5.68               & 37.01    & $-$3.22   \\           
NGC~4565 &    12 36 20.78 &    +25 59 15.6 &        9.7 & SA(s)b? spin    &       S1.9    & S                 & 136   & 7.46               & 38.22    & $-$3.79   \\           
NGC~4589 &    12 37 25.00 &    +74 11 30.9 &       30.0 & E2              &         L2    & L                 & 224.3 & 8.33               & 38.78    & $-$4.10   \\           
NGC~4605 &    12 39 59.38 &    +61 36 33.1 &        4.0 & SB(s)c pec      &           H   & H                 & 26.1  & 4.57               & 36.63    & $-$2.49   \\           
NGC~4618 &    12 41 32.85 &    +41 09 02.8 &        7.3 & SB(rs)m         &           H   & H                 & $<$54.6 & $<$5.86          & 37.97    & $>-$2.44  \\             
NGC~4648 &    12 41 44.39 &    +74 25 15.4 &       27.5 & E3              &           ALG & ALG               & 224.5 & 8.33                & $-$      & $-$      \\           
NGC~4631 &    12 42 08.01 &    +32 32 29.4 &        6.9 & SB(s)d spin     &           H   & H                 & $<$71.9 & $<$6.34         & 37.12    & $>-$3.77   \\        
NGC~4656 &    12 43 57.73 &    +32 10 05.3 &        7.2 & SB(s)m pec      &           H   & H                 & 70.4  & 6.31                & 37.93    & $-$2.93   \\          
NGC~4750 &    12 50 07.27 &    +72 52 28.7 &       26.1 & (R)SA(rs)ab     &         L1.9  & L                 & 136   & 7.46                 & 38.76    & $-$3.25   \\         
NGC~4725 &    12 50 26.58 &    +25 30 02.9 &       12.4 & SAB(r)ab pec    &       S2:     & S                 & 140   & 7.51                & 38.51    & $-$3.55   \\          
NGC~4736 &    12 50 53.06 &    +41 07 13.7 &        4.3 & (R)SA(r)ab      &         L2    &  L$^{c,r}$         & 112   & 7.12               & 37.33    & $-$4.08 \\            
NGC~4800 &    12 54 37.80 &    +46 31 52.2 &       15.2 & SA(rs)b         &         H     & H                 & 111   & 7.02$^{*}$          & 37.62    & $-$3.95  \\          
NGC~4793 &    12 54 40.62 &    +28 56 19.2 &       38.9 & SAB(rs)c        &           H   & H                 & 26.6  & 4.61                 & $<$38.84    & $<-$0.32  \\    
NGC~4826 &    12 56 43.64 &    +21 40 58.7 &        4.1 & (R)SA(rs)ab     &         T2    & L$^{b,r}$          & 96    & 6.85                & 37.92 & $-$3.48 \\              
NGC~5012 &    13 11 37.04 &    +22 54 55.8 &       40.4 & SAB(rs)c        &       T2      & L                 & 141.4 & 7.52                & 38.58    & $-$3.49  \\           
NGC~5033 &    13 13 27.47 &    +36 35 38.2 &       18.7 & SA(s)c          &         S1.5  &  L                & 151   & 7.64                & 39.34    & $-$2.85   \\          
NGC~5204 &    13 29 36.51 &    +58 25 07.4 &        4.8 & SA(s)m          &           H   & H                 & 39.9  & 5.32                & 36.58    & $-$3.29  \\           
NGC~5308 &    13 47 00.43 &    +60 58 23.4 &       32.4 & SA0- spin       &           ALG & ALG               & 249   & 8.51                & $-$      & $-$      \\           
NGC~5322 &    13 49 15.27 &    +60 11 25.9 &       31.6 & E3+             &         L2::  & L$^{s}$           & 232.2 & 8.39                & 38.20    & $-$4.74  \\           
NGC~5354 &    13 53 26.70 &    +40 18 09.9 &       32.8 & SA0 spin        &        T2/L2: & L                & 217.4 & 8.28                 & 38.61    & $-$4.22   \\          
NGC~5457 &    14 03 12.54 &    +54 20 56.2 &        5.4 & SAB(rs)cd       &           H   & H                 & 23.6  & 6.41$^{*}$          & 36.99    & $-$3.97   \\          
NGC~5473 &    14 04 43.23 &    +54 53 33.5 &       33.0 & SAB(s)0-:       &           ALG & ALG               & 220.5 & 8.30                & $-$      & $-$      \\           
NGC~5474 &    14 05 01.61 &    +53 39 44.0 &        6.0 & SA(s)cd pec     &           H   & H                 & 29    & 4.76                & 37.35    & $-$1.96  \\           
NGC~5485 &    14 07 11.35 &    +55 00 06.1 &       32.8 & SA0 pec         &         L2:   & L$^{t}$           & 207.5 & 8.19                 & 38.31    & $-$4.43  \\          
NGC~5548 &    14 17 59.53 &    +25 08 12.4 &       67.0 & (R')SA(s)0/a    &          S1.5 & S                 & 291   & 7.70$^{*}$          & 41.60    & $-$0.65  \\           
NGC~5585 &    14 19 48.20 &    +56 43 44.6 &        7.0 & SAB(s)d         &           H   & H                 & 42    & 5.41                & 37.68    & $-$2.28  \\           
NGC~5631 &    14 26 33.30 &    +56 34 57.5 &       32.7 & SA(s)0          &        S2/L2: & L$^{m}$           & 168.1 & 7.83                & 38.76    & $-$3.62  \\           
NGC~5678 &    14 32 05.61 &    +57 55 17.2 &       35.6 & SAB(rs)b        &         T2    & H                 & 132.8 & 7.42                & 38.27    & $-$3.70   \\          
NGC~6217 &    16 32 39.20 &    +78 11 53.4 &       23.9 & (R)SB(rs)bc     &         H     & H                 & 70.3  & 6.30                & 39.25    & $-$1.60  \\          
NGC~6207 &    16 43 03.75 &    +36 49 56.7 &       17.4 & SA(s)c          &           H   & H                 & 92.1  & 6.78                & 38.30    & $-$3.03   \\          
NGC~6236 &    16 44 34.65 &    +70 46 48.8 &       23.3 & SAB(s)cd        &           H   & H                 & 46.1  & 5.57                & 37.93    & $-$2.19   \\          
NGC~6340 &    17 10 24.85 &    +72 18 16.0 &       22.0 & SA(s)0/a        &         L2    & L                 & 143.9 & 7.56                & 38.31    & $-$3.80  \\           
NGC~6412 &    17 29 37.51 &    +75 42 15.9 &       23.5 & SA(s)c          &           H   & H                 & 49.9  & 5.71                & 37.59    & $-$2.67   \\          
NGC~6503 &    17 49 26.43 &    +70 08 39.7 &        6.1 & SA(s)cd         &        T2/S2: & L$^{r}$           & 46    & 6.30$^{*}$           & $-$      & $-$     \\           
NGC~6482 &    17 51 48.81 &    +23 04 19.0 &       52.3 & E:              &       T2/S2:: & L$^{b}$           & 310.4 & 8.90                 & $-$      & $-$      \\          
NGC~6643 &    18 19 46.41 &    +74 34 06.1 &       25.5 & SA(rs)c         &           H   & H                 & 95.4  & 6.84                & 37.52    & $-$3.87   \\          
NGC~6654 &    18 24 07.57 &    +73 10 59.6 &       29.5 & (R')SB(s)0/a    &           ALG & ALG               & 172.2 & 7.87                & $-$      & $-$      \\           
NGC~6689 &    18 34 50.25 &    +70 31 26.1 &       12.2 & SAd? spin       &           H   & L                 & 26    & 4.57                & 37.17    & $-$1.95   \\          
NGC~7080 &    21 30 01.95 &    +26 43 04.1 &       64.1 & SB(r)b          &           H & H:                  & 95.3  & 6.84                 & $-$      & $-$      \\          
\hline
\hline
\end{longtable}
\end{center}
\vspace*{-1.1cm}\fontsize{8}{7}\selectfont Column description: (1)
source name; (2)-(3) RA and DEC position
(J2000) from NED, using optical or infrared images; (4) distance (Mpc)
from \citet{ho97a}; (5)
 morphological galaxy type given from RC3
\citep{devaucouleurs91}; (6) optical spectroscopic classification
based on \citet{ho97a}: H=H{\sc ii}, S=Seyfert, L=LINER, T=Transition
object, and ALG=Absorption line galaxy. The number attached to the
class letter designates the AGN type (between 1 and 2); quality
ratings are given by ':' and '::' for uncertain and highly uncertain
classification, respectively. Two classifiations are given for some
ambiguous cases, where the first entry corresponds to the adopted
choice; (7) optical spectroscopic classification based on BPT diagrams
and from the literature. See the notes for the classification based on
the literature; (8) stellar velocity dispersion (\kms) from
\citet{ho09}; (9) logarithm of the SMBH mass (M$_{\odot}$) determined
based on stellar velocity dispersions \citep{tremaine02} and the
galaxies marked with $^{*}$ have direct BH mass measurements from
\citet{vanderbosch16}. ; (10) logarithm of the [O~III] luminosities from \citet{ho97a} or from
the same reference used for the optical classification; (11) logarithm of the Eddington
ratio, i.e. ratio between the bolometric and Eddington luminosity.
\\ Notes: letters correspond to following publications: $a$
\citet{keel83} $b$ \citet{vandebosch15} $c$ \citet{moustakas06} $d$
\citet{florido12} $e$ \citet{buttiglione10alias} $f$ \citet{gavazzi13}
$g$ \citet{heckman80} $h$ \citet{balmaverde13}; $i$ SDSS; $j$
\citet{gavazzi18} $k$ \citet{cazzoli18} $l$ \citet{shields07} $m$
\citet{nyland16} $n$ \citet{serra18} $o$ \citet{wegner03} $p$
\citet{pismis01} $q$ \citet{kennicutt92} $r$ \citet{lira07} $s$
\citet{baldi09} $t$ \citet{garcia15}.

%\vspace{1cm}
\normalfont\normalsize

\begin{multicols}{2}


 
\end{multicols}


%\end{minipage} 
%\citet{annibali10};  ; 
%\citet{cidfernandes05};  \citet{goulding09}; 
%\citet{moustakas06};  \citet{trippe10}; \citet{cappellari01};
% SDSS;  \citet{dale06};  \citet{balmaverde14}; 
% \citet{rampazzo95}; \citet{leech89}; 
%\citet{perez00};  , \citet{bower92}; 
%\citet{falco99}, \citet{sarzi06}.  
%\twocolumn \normalfont\normalsize


\twocolumn \normalfont\normalsize

